Predicting Multi-Codebook Vector Quantization Indexes for Knowledge Distillation

Knowledge distillation(KD) is a common approach to improve model performance in automatic speech recognition (ASR), where a student model is trained to imitate the output behaviour of a teacher model. However, traditional KD methods suffer from teacher label storage issue, especially when the training corpora are large. Although on-the-fly teacher label generation tackles this issue, the training speed is significantly slower as the teacher model has to be evaluated every batch. In this paper, we reformulate the generation of teacher label as a codec problem. We propose a novel Multi-codebook Vector Quantization (MVQ) approach that compresses teacher embeddings to codebook indexes (CI). Based on this, a KD training framework (MVQ-KD) is proposed where a student model predicts the CI generated from the embeddings of a self-supervised pre-trained teacher model. Experiments on the LibriSpeech clean-100 hour show that MVQ-KD framework achieves comparable performance as traditional KD methods (l1, l2), while requiring 256 times less storage. When the full LibriSpeech dataset is used, MVQ-KD framework results in 13.8% and 8.2% relative word error rate reductions (WERRs) for non -streaming transducer on test-clean and test-other and 4.0% and 4.9% for streaming transducer. The implementation of this work is already released as a part of the open-source project icefall.

==> text_prev/abs.tex <==
\begin{abstract}
% Given a limited amount of acoustic data with transcriptions, 
Self-supervised pre-training is an effective approach to leveraging a large amount of unlabelled data to boost the performance of automatic speech recognition (ASR) systems. 
% Self-supervised learning ASR models have the advantage of yielding high recognition accuracy given only limited labelled data.
% To fully exploit unlabelled data, a pre-trained model usually has hundreds of millions of parameters.
However, it is impractical to serve large pre-trained models for real-world ASR applications.
% For real-world ASR applications, serving large pre-trained models  would be impractical.
% Therefore, it is desirable to take advantage of the large pre-trained models to yield a high-performing speech recogniser but with limited model size.
Therefore, it is desirable to have a much smaller model while retaining the performance of the pre-trained model.
% However, their enormous model size makes them inappropriate for real ASR applications.
% Knowledge distillation, a model compression technique that trains a small student model to match the output distributions of the large teacher model, can also make use of unlabelled data.
% making it also applicable when unlabelled data is provided.
In this paper, we propose a simple knowledge distillation (KD) loss function for neural transducers that focuses on the one-best path in the output probability lattice under both the streaming and non-streaming setups, which allows the small student model to approach the performance of the large pre-trained teacher model.
% In this paper, we combine the merits of self-supervised pretraining and knowledge distillation to obtain a small well-performing RNN-Transducer (RNN-T) model with limited labelled data.
% To distil knowledge on RNN-T effectively, we propose a novel distillation loss as an auxiliary task for RNN-T models that focuses on the one-best path in the RNN-T output lattice.
% We also modify our distillation proposal so that it can be easily applied on streaming RNN-T models.
% Experiment results on LibriSpeech dataset suggest that our distillation proposal is both memory-efficient and effective.
%Experiments on the LibriSpeech dataset show that despite being more than 10 times smaller than the teacher model, the non-streaming student achieves up to 37.2\% and 50.4\% relative word error rate reductions (WERRs) on test-clean and test-other sets. For the streaming student model, up to 19.7\% and 38.5\% WERRs are observed. The performance of the student model can be further improved if the distillation targets are generated by applying language model shallow fusion with the teacher model.
Experiments on the LibriSpeech dataset show that despite being more than 10 times smaller than the teacher model, the proposed loss results in relative word error rate reductions (WERRs) of 11.4\% and 6.8\% on test-other set for non-streaming and streaming student models compared to the baseline transducers trained without KD using the labelled 100-hour clean data. With additional 860-hour unlabelled data for KD, the WERRs increase to 50.4\% and 38.5\% for non-streaming and streaming students. If language model shallow fusion is used for producing distillation targets, further improvement on the student model is observed.

% the student models achieve 11.4\% (non-streaming) and 6.8\% (streaming) relative word error rate reductions (WERRs) while only using the 100h labelled subset for knowledge distillation (KD). Furthermore, the student model achieves 50.4\% (non-streaming) and 38.6\% (streaming) WERRs when an additional 860h of unlabelled data is used for KD.
% Without incorporating extra unlabelled data, we obtain WER reduction of 11.4\% and 6.8\% for non-streaming and streaming RNN-T models respectively on 100h experiments. By incorporating the rest 860h as unlabelled data, our KD proposal achieves a WER reduction of 50.4\% and 38.6\% on test-other for non-streaming and streaming RNN-T models respectively on the same amount of labelled data (100h).
\end{abstract}

\begin{keywords}
knowledge distillation, neural transducer, ASR
\end{keywords}

==> text_prev/abs_new.tex <==
\begin{abstract}
% Given a limited amount of acoustic data with transcriptions, 
Self-supervised pre-training is an effective approach to leveraging a large amount of unlabelled data to boost the performance of automatic speech recognition (ASR) systems. 
% Self-supervised learning ASR models have the advantage of yielding high recognition accuracy given only limited labelled data.
% To fully exploit unlabelled data, a pre-trained model usually has hundreds of millions of parameters.
However, it is impractical to serve large pre-trained models for real-world ASR applications.
% For real-world ASR applications, serving large pre-trained models  would be impractical.
% Therefore, it is desirable to take advantage of the large pre-trained models to yield a high-performing speech recogniser but with limited model size.
Therefore, it is desirable to have a much smaller model while retaining the performance of the pre-trained model.
% However, their enormous model size makes them inappropriate for real ASR applications.
% Knowledge distillation, a model compression technique that trains a small student model to match the output distributions of the large teacher model, can also make use of unlabelled data.
% making it also applicable when unlabelled data is provided.
In this paper, we propose a simple knowledge distillation (KD) loss function for neural transducers that focuses on the one-best path in the output probability lattice under both the streaming and non-streaming setups, which allows the small student model to approach the performance of the large pre-trained teacher model.
% In this paper, we combine the merits of self-supervised pretraining and knowledge distillation to obtain a small well-performing RNN-Transducer (RNN-T) model with limited labelled data.
% To distil knowledge on RNN-T effectively, we propose a novel distillation loss as an auxiliary task for RNN-T models that focuses on the one-best path in the RNN-T output lattice.
% We also modify our distillation proposal so that it can be easily applied on streaming RNN-T models.
% Experiment results on LibriSpeech dataset suggest that our distillation proposal is both memory-efficient and effective.
%Experiments on the LibriSpeech dataset show that despite being more than 10 times smaller than the teacher model, the non-streaming student achieves up to 37.2\% and 50.4\% relative word error rate reductions (WERRs) on test-clean and test-other sets. For the streaming student model, up to 19.7\% and 38.5\% WERRs are observed. The performance of the student model can be further improved if the distillation targets are generated by applying language model shallow fusion with the teacher model.
Experiments on the LibriSpeech dataset show that despite being more than 10 times smaller than the teacher model, the proposed loss results in relative word error rate reductions (WERRs) of \textcolor{blue}{11.5\%} and 6.8\% on test-other set for non-streaming and streaming student models compared to the baseline transducers trained without KD using the labelled 100-hour clean data. With additional 860-hour unlabelled data for KD, the WERRs increase to \textcolor{blue}{48.2\%} and 38.5\% for non-streaming and streaming students. If language model shallow fusion is used for producing distillation targets, further improvement on the student model is observed.

% the student models achieve 11.4\% (non-streaming) and 6.8\% (streaming) relative word error rate reductions (WERRs) while only using the 100h labelled subset for knowledge distillation (KD). Furthermore, the student model achieves 50.4\% (non-streaming) and 38.6\% (streaming) WERRs when an additional 860h of unlabelled data is used for KD.
% Without incorporating extra unlabelled data, we obtain WER reduction of 11.4\% and 6.8\% for non-streaming and streaming RNN-T models respectively on 100h experiments. By incorporating the rest 860h as unlabelled data, our KD proposal achieves a WER reduction of 50.4\% and 38.6\% on test-other for non-streaming and streaming RNN-T models respectively on the same amount of labelled data (100h).
\end{abstract}

\begin{keywords}
knowledge distillation, neural transducer, ASR
\end{keywords}

==> text_prev/background.tex <==
\presec
\section{Self-supervised Pre-training for E2E ASR}
\postsec
\label{sec:background}

% Here, we first set up notations by giving a brief review of wav2vec 2.0 self-supervised learning approach and the RNN-T architecture. 

% \presec
\subsection{wav2vec 2.0 for Self-Supervised Pre-training}
\postsec
\label{sec:w2v}
Self-supervised learning for E2E ASR has shown promising results in the last few years~\cite{baevski2019vqw2v2, jiang2019improving, baevski2020wav2vec}. Among these methods, wav2vec 2.0 (w2v2) is one of the most promising and effective frameworks.
% Inspired by masked language modelling in BERT~\cite{devlin2018bert}, w2v2 extends this idea to ASR pre-training.
The raw speech waveform $\mathbf{w}$ is first processed by a convolutional neural network feature extractor $\mathcal{M}$ to generate latent speech representations $\mathcal{M}(\mathbf{w})=\mathbf{z}_{1:T}$, which are then sent to a Transformer network $\mathcal{N}$ to generate contextualised speech representations $\mathcal{N}(\mathbf{z}_{1:T}) = \mathbf{c}_{1:T}$.
A quantisation module $\mathcal{Q}$ discretises the latent speech representation to $\mathbf{q}_t$.
% A quantisation module $\mathcal{Q}$ using product quantisation~\cite{jegou2010productquant} and gumbel softmax~\cite{jang2016gumbelsoftmax} is also incorporated in the training process, which transforms the latent speech representation $\mathbf{z}_t$ to $\mathbf{q}_t$.
Pre-training is carried out by predicting the correct quantised representations of the masked latent speech representations from a set of distractors. % For example, if the latent speech representation $\mathbf{z}_t$ at timestamp $t$ is masked, the transformer output $\mathbf{c}_t$ at timestamp $t$ should resemble $\mathcal{Q}(\mathbf{z}_t) = \mathbf{q}_t$ as much as possible. 
This training objective for each $\mathbf{z}_t$ can be expressed with a contrastive loss function \eqndot{w2v2}, where $Q_t$ is a set consisting of the correct quantisation $\mathbf{q}_t$ and other distractors, $\kappa$ is the temperature and $\textsc{sim}$ denotes a similarity measure. An additional quantisation diversity loss is added to construct the final loss during pre-training.
\begin{align}
    \mathcal{L}_{\text{contrastive}} = -\log \frac{\exp(\textsc{sim}(\mathbf{c}_t, \mathbf{q}_t)/\kappa)}{\sum_{\mathbf{q}\in Q_t}\exp(\textsc{sim}(\mathbf{c}_t,\mathbf{q})/\kappa)}.
    \label{eqn:w2v2}
\end{align}

The pre-trained model is used to initialise the encoder in an E2E ASR model. The encoder is then fine-tuned together with additional output layers or decoders using labelled data for ASR. Although the original pre-trained models are fine-tuned with the CTC objective~\cite{baevski2020wav2vec}, they can also be used to initialise transducer models~\cite{Zhang2020PushingTL}.
% After pre-training, the model will be integrated as encoder in an ASR model and fine-tuned with labelled data to perform ASR tasks. Although the w2v2 model is experimented under a CTC framework~\cite{baevski2020wav2vec}, it can be easily extended to be used in RNN-T architectures, which will be reviewed below in \sectdot{rnnt}.

\presec
\subsection{Neural Transducer Model}
\postsec
\label{sec:rnnt}
CTC~\cite{graves2006CTC} is one of the earliest frameworks for E2E ASR. Since assuming the output tokens at different timestamps are conditionally independent is not realistic for ASR, the RNN transducer was proposed later to address this limitation~\cite{graves2012RNNT}. More recently, the encoder of the transducer is no longer limited to RNNs for improved performance, such as Transformer transducers~\cite{Zhang2020TransformerTA} and Conformer transducers~\cite{gulati2020conformer}.
% E2E ASR was first introduced under the framework of Connectionist Temporal Classification (CTC)~\cite{graves2006CTC}, where the generation of output token at different time stamps is independent. To model dependency between each prediction, the RNN-T architecture was introduced~\cite{graves2012RNNT}.
A neural transducer model consists of an encoder $\mathcal{F}$, a prediction network $\mathcal{G}$ and a joint network $\mathcal{J}$. During training, given an input feature sequence $\mathbf{X} = \mathbf{x}_{1:T}$ of length $T$, the encoder $\mathcal{F}$ extracts the latent representations $\mathbf{f}_{1:T}$. The prediction network predicts the next symbol $y_{u}$ given all previous symbols ${y_{1:u-1}}$ for $u=1,\dots,U$, similar to a language model. The output from the prediction network $\mathcal{G}(\mathbf{y}) = \mathbf{g}_{1:U}$ is then fed to $\mathcal{J}$ together with $\mathbf{f}_{1:T}$ to generate an output distribution lattice $\mathbf{Z}$ of dimension $K \times T\times U$, where $K$ is the output vocabulary size. The probability $p(k|t,u)$ of emitting token $k$ at node $(t,u)$ in $\mathbf{Z}$ is then defined as the $k$-th entry in the vector obtained after applying softmax operation on $\mathbf{Z}(t,u)$. The training of transducer is done by maximising the probability $p(\mathbf{y}|\mathbf{X})$, which can be efficiently computed with a forward-backward algorithm on the lattice $\mathbf{Z}$~\cite{graves2012RNNT}.

Neural transducers generally outperform CTC models due to their ability to model the dependency across the output tokens. As the decoding procedure is frame-synchronous, transducers are suitable for streaming applications given the encoder only has a limited exposure of future acoustic context~\cite{rao2017exploring, he2019streaming}.
% The decoder's capability of modelling output dependency distinguish the RNN-T model from CTC models and leads to better performance. Also, the sequential manner of output generation makes RNN-T models a suitable candidate for streaming applications~\cite{rao2017exploring, he2019streaming}.
% For streaming RNN-T models, the encoder should be causal: no future information should be available for making the current prediction.
% Architectures supporting streaming transducer models include uni-directional recurrent layers (for example LSTM layer~\cite{hochreiter1997lstm}) or masked attention~\cite{vaswani2017transformer}. Due to the lack of future information during prediction, the streaming transducer model's performance tends to be much worse than their non-streaming counterparts~\cite{battenberg2017exploring}.

==> text_prev/conclusion.tex <==
\presec
\section{Conclusion}
\postsec
\label{sec:conclusion}
In this paper, we propose a simple and efficient knowledge distillation (KD) loss for neural transducers using the full distribution along the one-best alignment of the output distribution lattice. This approach can be easily extended to distil knowledge from a non-streaming transducer to a streaming one. We showcased the effectiveness of the proposed approach by distilling knowledge from a non-streaming teacher model initialised from a large self-supervised pre-trained to both non-steaming and streaming student models that are more than 10 times smaller. Experiments also show that the performance of the student model can be greatly improved by having more unlabelled data for KD or augmenting the distillation targets by language model shallow fusion.
% On LibriSpeech test-clean and test-other datasets, the non-streaming student model can achieve 54.4\% relative word error rate reduction (WERR) and the streaming student model can achieve 38.5\% WERR with the best setup compared to the baseline student Conformer transducer trained without KD.
With better teacher models or more unlabelled data, the student models are expected to reach better performance. In the future, we will explore how to best transfer information from an external language model to the student model, and how to distil knowledge more effectively from a non-streaming teacher to a streaming student.
% In this paper, we carried out KD to compress self-supervised ASR model (wav2vec 2.0) for constructing a small COnformer transducer models with good performance. We proposed a novel and efficient RNN-T distillation loss based on the one-best path in the RNN-T output lattice which is applicable to both non-streaming and streaming RNN-T models. KD experiments on clean-100h subset achieves a WERR of 11.4\% (non-streaming) and 6.8\% (streaming).  By utilising extra 860h data as unlabelled data set, our KD proposal further improves the student model performance, resulting in a WERR of 50.4\% (non-streaming) and 38.6\% (streaming) without increasing the amount of labelled data. 

% Experiments on the LibriSpeech dataset show that despite being more than 10 times smaller than the teacher model, the proposed distillation loss results in relative word error rate reductions (WERRs) of 11.4\% and 6.8\% on test-other set for non-streaming and streaming student models compared to the baseline transducers trained without distillation using the labelled 100-hour clean data. With additional 860-hour unlabelled data for KD, the WERRs increase to 50.4\% and 38.5\% for non-streaming and streaming students.

==> text_prev/exp.tex <==
\presec
\section{Experimental Results}
\postsec
\label{sec:results}
% Two sets of knowledge distillation experiments are carried out to investigate the effectiveness of our proposed distillation loss. The first set of experiments are performed on the clean-100h labelled data set to examine the effectiveness of our proposed distillation loss. The full-lattice distillation loss~\cite{panchapagesan2021fulllatticernntkd} is also implemented and a comparison is made. In the second set of experiments, the rest 860h of LibriSpeech dataset is as unlabelled data to form a semi-supervised learning scenario to further exploit the potential of our distillation loss.

% \presec
\subsection{Baselines}
\postsec
In \tbl{ref models}, word error rate (WER) of both the fine-tuned w2v2 models and the baseline conformer models trained on LibriSpeech 100-hour subset are reported. The fine-tuning configurations of the teacher model follow \cite{baevski2020wav2vec}. Although our implementation shares the same pre-trained encoder as \cite{baevski2020wav2vec} (\textsc{Base}\footnote{\url{https://github.com/pytorch/fairseq/tree/main/examples/wav2vec}}), the performance is better because our fine-tuned w2v2 model is a transducer model with BPE modelling units instead of a CTC model with grapheme units~\cite{baevski2020wav2vec}. For the baseline Conformer-S models, SpecAugment~\cite{park2019specaugment} is used during training, which has 2 frequency masks with $F=27$ and 10 time masks with a maximum time-mask ratio of 0.05.
\begin{table}[ht]
    \pretbl
    \centering
    \begin{tabular}{lrrrr}
        \toprule
        \multirow{2}{*}{Models}    & \multicolumn{2}{c}{dev}   & \multicolumn{2}{c}{test}  \\
        \cmidrule(lr){2-3}  \cmidrule(lr){4-5}
        & \multicolumn{1}{c}{clean} & \multicolumn{1}{c}{other} & \multicolumn{1}{c}{clean} & \multicolumn{1}{c}{other} \\ 
        \midrule
        w2v2 CTC (\cite{baevski2020wav2vec})   &  6.1 & 13.5 &  6.1 & 13.3\\
        w2v2 transducer (ours)                        &  5.1 & 12.2  &  5.2 & 11.8 \\
        \;\;\;\; + LM shallow fusion                   &  4.2 & 10.4 &  4.3 & 10.1\\
        \midrule
        Conformer-S (non-streaming)              &  8.2 & 22.4 &  8.6 & 22.8\\
        Conformer-S (streaming)                  & 11.2 & 28.4 & 12.2 & 29.6\\
        \bottomrule
    \end{tabular}
    \caption{WERs of the w2v2 models and the baseline small Conformer models trained on LibriSpeech 100-hour subset. Our fine-tuned w2v2 transducer will be used as the teacher model.}
    \label{tab:ref models}
    \posttbl
\end{table}

% Our fine-tuned w2v2 transducer model with a sub-sampling module outperforms the original w2v2 CTC model. This confirms the benefits of using transducer models as a better teacher model is more likely to generate better distillation label, which tends to lead to better student models.
As expected, the w2v2 transducer has much lower WERs than the non-streaming Conformer-S model as it benefits from self-supervised pre-training and a larger model size. To have a streaming transducer, an attention mask is added to remove the contribution of future frames in the encoder and the 1D-convolution is changed to 1D causal convolution to only attend to previous frames. Consequently, the performance of Conformer-S drops significantly.
% ~\cite{oord2016wavenet}
% As expected, a large performance gap between the baseline Conformer model and the teacher w2v2 model is observed. From now on, all distillation labels will be generated from this teacher w2v2 transducer model.

In the following experiments, the w2v2 transducer (second row in \tbl{ref models}) will be used as the teacher model. The student transducer model with the same architecture as Conformer-S will try to approach the performance of the teacher model. For both the non-streaming and the streaming setups, the 100-hour labelled training data is used first to verify the proposed KD approach. Then, the remaining 860-hour training data is used as unlabelled data to further improve the student models.
% Beam sizes of 20 and 8 are used for w2v2-based models and Conformer-based model.

\presec
\subsection{KD for Non-Streaming Transducers}
\postsec
\label{ssec:non-streaming_trans}
Two KD training strategies are investigated for the proposed distillation loss. The first strategy (ST1) trains the student transducer model from scratch using \eqndot{kd full loss}. The second strategy (ST2) initialises the student model from a model trained on ground truth or pseudo transcriptions and then uses the proposed loss in \eqndot{kd full loss} for fine-tuning.
\begin{table}[ht]
    \pretbl
    \centering
    \begin{tabular}{lrrrr}
        \toprule
        \multirow{2}{*}{Transducer models}    & \multicolumn{2}{c}{dev}   & \multicolumn{2}{c}{test}  \\
        \cmidrule(lr){2-3}  \cmidrule(lr){4-5}
        & \multicolumn{1}{c}{clean} & \multicolumn{1}{c}{other} & \multicolumn{1}{c}{clean} & \multicolumn{1}{c}{other} \\ 
        \midrule
        \multicolumn{5}{l}{\textbf{Reference models: 100h labelled}}\\
        w2v2 transducer (teacher) & 5.1 & 12.2 & 5.2 & 11.8\\
        Conformer-S (baseline)     & 8.2 & 22.4 & 8.6 & 22.8\\
        \midrule
        \multicolumn{5}{l}{\textbf{Student models: 100h labelled}}\\
        $\lambda=0.001$, collapsed dist.\cite{panchapagesan2021fulllatticernntkd} & 7.1 & 20.7 & 7.5 & 20.9\\
        $\lambda=0.1$, ST1       & 7.1 & 19.8 & 7.6 & 20.5 \\
        $\lambda=0.1$, ST2       & 7.1 & 19.7 & 7.5 & 20.2 \\
        $\lambda=0.1$, ST2 [+LM] & 6.9 & 19.6 & 7.4 & 20.0 \\
        \midrule
        \multicolumn{5}{l}{\textbf{Student models: 100h labelled + 860h unlabelled}}\\
        $\lambda=0.0$            & 5.5 & 11.5 & 5.6 & 11.9 \\
        $\lambda=0.0$ [+LM]      & 4.7 & 10.4 & 4.8 & 10.9 \\
        $\lambda=0.1$, ST1       & 5.5 & 11.3 & 5.5 & 11.7 \\
        $\lambda=0.1$, ST2       & 5.3 & 10.9 & 5.4 & 11.3 \\
        $\lambda=0.1$, ST2 [+LM] & 4.6 & 10.1 & 4.8 & 10.4 \\
        \bottomrule
    \end{tabular}
    \caption{WERs of non-streaming transducer models. $\lambda$ is the weight of KD loss. [+LM] means either the teacher output distributions or the pseudo transcriptions are obtained after LM shallow fusion.}
    \label{tab:non-streaming KD}
    \posttbl
\end{table}
% KD experiments are first carried out on non-streaming transducer models.
% For ST2, we initialise the model from baseline model in \tbl{ref models} in 100h experiments and the model trained with 100h ground truth and 860 pseudo transcription data in 960h experiments.
% ST1 means the student model is trained from scratch. ST2 means the student model is initialised from a model trained on ground truth or pseudo transcriptions. 

Five key observations can be made from \tbl{non-streaming KD}.
First, for student models trained from 100h labelled data, the proposed distillation loss using the full distribution on the one-best alignment slightly outperforms KD using a collapsed distribution on the whole lattice~\cite{panchapagesan2021fulllatticernntkd}.
Secondly, for student models trained from 100h labelled data and 860h unlabelled data, the proposed KD method yields lower WERs than simply using the pseudo transcriptions ($\lambda=0.0$) for the unlabelled data because the output distribution carries more information from the teacher to the student than the pseudo transcriptions.
Thirdly, ST2 has marginally lower WERs than ST1 for both the 100h and the 960h setups. As a result, ST2 will be used for the streaming experiments in \ssectdot{streaming_trans}.
Fourthly, the relative WER reductions (WERRs) on test-clean and test-other are 12.8\% and 11.4\% by using the proposed KD loss compared with the baseline. They increase to 37.2\% and 50.4\% when an additional 860h of unlabelled data is used for KD.
Lastly, to distil the knowledge from both the teacher model and the LM together, shallow fusion is used to generate the pseudo transcriptions on the unlabelled data and to augment the output distributions. This leads to WERRs of 14.0\% and 12.3\% for the 100h setup compared with the baseline. After incorporating 860h unlabelled data, they improve to 44.2\% and 54.4\%.

% To prevent model from diverging and catastrophic forgetting, the fine-tuning learning rate in ST2 is set very small.
%Note that the student model pre-training in the second strategy is only performed on clean-100h dataset to ensure only limited resource of labelled data is used. 
% In clean-100h experiments, the result of our implementation of \cite{panchapagesan2021fulllatticernntkd} is also included for comparison. For 960h experiments, the pseudo transcriptions decoded from the teacher transducer model and one-best path of 860h unlabelled data are collected. The WERs are shown in \tbl{non-streaming KD}. Among the two KD training strategies, ST2 yields a better results in both 100h and 960h experiments, showing the necessity of a good initialisation for KD. Therefore, only ST2 will be adopted in the following experiments. Compared with results of the distillation loss in~\cite{panchapagesan2021fulllatticernntkd}, our method achieves a higher WER reduction on the more challenging other sets. Compared with the baseline student conformer models, a relative WER reduction of 12.8\% and 11.4\% can be observed on test-clean and test-other using our proposed distillation loss together with ST2 on clean-100h. 

% After including more unlabelled data, the performance gap between the teacher model and the student model is further closed. By fine-tuning the model trained with 100h ground truth and 860h pseudo transcription without KD, our distillation proposal further improves the WER, achieving a relative reduction of 37.2\% and 50.4\% (see bottom row in \tbl{non-streaming KD}) compared to the baseline model. We also see that the WER improvement brought by KD is less obvious in 960h experiments than in 100h experiments. This is due to the reason that the teacher model is only trained on clean-100h, thus the quality of both the pseudo transcription and one-best distillation label is limited. A further WER improvement is observed after incorporating LM information in the distillation label.

\presec
\subsection{KD for Streaming Transducers}
\postsec
\label{ssec:streaming_trans}
% ST2 means the student model is initialised from a model trained on ground truth or pseudo transcriptions. [+LM] means either the output distributions or the pseudo transcriptions are obtained after LM shallow fusion.
By introducing the parameter $\tau$ for delaying the alignment, the proposed one-best distillation loss is applied to train streaming student models.
% The modified one-best distillation loss is then applied to streaming transducer models. To ensure that no future information is used during prediction, the original Conformer block is modified. An attention mask is added to remove the contribution of future frames when calculating the attention score and the 1D-convolution is changed to 1D causal convolution to only attend to previous frames \cite{oord2016wavenet}.
As before, the distillation targets are still generated from the non-streaming teacher w2v2 transducer. When the streaming student model is trained to match the alignment of the non-streaming teacher, \ie when $\tau=0$, the WERs of the student model is even higher than the baseline due to a lack of future context. After observing the one-best alignment of a streaming transducer can be multiple steps behind the one-best alignment of a non-streaming transducer, the WERs of $\tau=6$ and $\tau=7$ (equivalent to a look-ahead of 240 ms and 280 ms) are shown in \tbl{streaming KD}. Although more delay steps result in improved WERs, the latency of the ASR model is also increased. Nevertheless, setting a sensible value of $\tau$ is key to train a student model using KD.
% Three $\tau$s of 0, 6 and 7 are experimented after observing the delay of posterior peak between w2v2 transducer and streaming student models in 100h experiments. WER results are shown in \tbl{streaming KD}. As expected, the KD results are very sensitive to the selection of $\tau$. The lowest WERs are obtained using $\tau=7$, which is also around the average delay of posterior peak between teacher and student lattice. Interestingly, if no time-shift is applied (i.e $\tau$=0), the student model after KD performs much worse than the streaming baseline. This again proves the significance of time-shift operation in streaming transducer distillation.
Compared with the streaming baseline, the proposed distillation approach achieves WERRs of 7.4\% and 6.8\% on test-clean and test-other in 100h experiments. After using the additional 860h unlabelled data, the student model trained with KD outperforms the one only trained with pseudo transcriptions, which increases WERRs to 19.7\% and 38.5\% \wrt the streaming baseline.
%After using the LM-augmented distillation targets, the WERs of the streaming student transducer are \% and \% lower than the baseline.
\begin{table}[ht]
    \pretbl
    \centering
    \begin{tabular}{lrrrr}
        \toprule
        \multirow{2}{*}{Transducer models}    & \multicolumn{2}{c}{dev}   & \multicolumn{2}{c}{test}  \\
        \cmidrule(lr){2-3}  \cmidrule(lr){4-5}
        & \multicolumn{1}{c}{clean} & \multicolumn{1}{c}{other} & \multicolumn{1}{c}{clean} & \multicolumn{1}{c}{other} \\ 
        \midrule
        \multicolumn{5}{l}{\textbf{Reference models: 100h labelled}}\\
        w2v2 transducer (teacher) &  5.1 & 12.2 &  5.2 & 11.8\\
        Conformer-S (baseline)         & 11.2 & 28.4 & 12.2 & 29.6\\
        \midrule
        \multicolumn{5}{l}{\textbf{Student models: 100h labelled}}\\
        $\lambda=0.1$, $\tau$=0, ST2 & 20.2 & 39.7& 20.5 & 41.4 \\
        $\lambda=0.1$, $\tau$=6, ST2 & 10.7 & 26.7& 11.3 & 28.0 \\
        $\lambda=0.1$, $\tau$=7, ST2 & 10.6 & 26.4& 11.3 & 27.6\\
        % $\lambda=0.1$, $\tau$=7, ST2 [+LM] & 10.4 & 26.5 & 11.1 & 27.4 \\
        \midrule
        \multicolumn{5}{l}{\textbf{Student models: 100h labelled + 860h unlabelled}}\\
        $\lambda=0.0$                & 9.5  & 19.3 & 10.6 & 19.7  \\
        % $\lambda=0.0$ [+LM]          & 9.1  & 18.4 & 10.3 & 18.5 \\
        $\lambda=0.1$, $\tau$=7, ST2 & 9.2  & 18.3 & 9.8  & 18.2 \\
        % $\lambda=0.1$, $\tau$=7, ST2 [+LM] & 8.9 & 18.7 & 9.7 & 18.7 \\
        \bottomrule
    \end{tabular}
    \caption{WERs of streaming transducer models. $\lambda$ is the weight of KD loss. $\tau$ is the number of delayed steps for the one-best alignment from the teacher model.}
    \label{tab:streaming KD}
    \posttbl
\end{table}
% [+LM] means either the output distributions or the pseudo transcriptions are obtained after LM shallow fusion.

% Although the streaming student has a much lower baseline than the non-streaming student, the relative improvement for the streaming student model is less. 


==> text_prev/exp_new.tex <==
\presec
\section{Experimental Results}
\postsec
\label{sec:results}
% Two sets of knowledge distillation experiments are carried out to investigate the effectiveness of our proposed distillation loss. The first set of experiments are performed on the clean-100h labelled data set to examine the effectiveness of our proposed distillation loss. The full-lattice distillation loss~\cite{panchapagesan2021fulllatticernntkd} is also implemented and a comparison is made. In the second set of experiments, the rest 860h of LibriSpeech dataset is as unlabelled data to form a semi-supervised learning scenario to further exploit the potential of our distillation loss.

% \presec
\subsection{Baselines}
\postsec
In \tbl{ref models}, word error rate (WER) of both the fine-tuned w2v2 models and the baseline conformer models trained on LibriSpeech 100-hour subset are reported. The fine-tuning configurations of the teacher model follow \cite{baevski2020wav2vec}. Although our implementation shares the same pre-trained encoder as \cite{baevski2020wav2vec} (\textsc{Base}\footnote{\url{https://github.com/pytorch/fairseq/tree/main/examples/wav2vec}}), the performance is better because our fine-tuned w2v2 model is a transducer model with BPE modelling units instead of a CTC model with grapheme units~\cite{baevski2020wav2vec}. For the baseline Conformer-S models, SpecAugment~\cite{park2019specaugment} is used during training, which has 2 frequency masks with $F=27$ and 10 time masks with a maximum time-mask ratio of 0.05.
\begin{table}[ht]
    \pretbl
    \centering
    \begin{tabular}{lrrrr}
        \toprule
        \multirow{2}{*}{Models}    & \multicolumn{2}{c}{dev}   & \multicolumn{2}{c}{test}  \\
        \cmidrule(lr){2-3}  \cmidrule(lr){4-5}
        & \multicolumn{1}{c}{clean} & \multicolumn{1}{c}{other} & \multicolumn{1}{c}{clean} & \multicolumn{1}{c}{other} \\ 
        \midrule
        w2v2 CTC (\cite{baevski2020wav2vec})   &  6.1 & 13.5 &  6.1 & 13.3\\
        w2v2 transducer (ours)                        &  5.1 & 12.2  &  5.2 & 11.8 \\
        \;\;\;\; + LM shallow fusion                   &  4.2 & 10.4 &  4.3 & 10.1\\
        \midrule
        \rowcolor{LightCyan}
        Conformer-S (non-streaming)              & 7.5 & 20.9 & 8.0 & 21.8\\
        Conformer-S (streaming)                  & 11.2 & 28.4 & 12.2 & 29.6\\
        \bottomrule
    \end{tabular}
    \caption{WERs of the w2v2 models and the baseline small Conformer models trained on LibriSpeech 100-hour subset. Our fine-tuned w2v2 transducer will be used as the teacher model.}
    \label{tab:ref models}
    \posttbl
\end{table}

% Our fine-tuned w2v2 transducer model with a sub-sampling module outperforms the original w2v2 CTC model. This confirms the benefits of using transducer models as a better teacher model is more likely to generate better distillation label, which tends to lead to better student models.
As expected, the w2v2 transducer has much lower WERs than the non-streaming Conformer-S model as it benefits from self-supervised pre-training and a larger model size. To have a streaming transducer, an attention mask is added to remove the contribution of future frames in the encoder and the 1D-convolution is changed to 1D causal convolution to only attend to previous frames. Consequently, the performance of Conformer-S drops significantly.
% ~\cite{oord2016wavenet}
% As expected, a large performance gap between the baseline Conformer model and the teacher w2v2 model is observed. From now on, all distillation labels will be generated from this teacher w2v2 transducer model.

In the following experiments, the w2v2 transducer (second row in \tbl{ref models}) will be used as the teacher model. The student transducer model with the same architecture as Conformer-S will try to approach the performance of the teacher model. For both the non-streaming and the streaming setups, the 100-hour labelled training data is used first to verify the proposed KD approach. Then, the remaining 860-hour training data is used as unlabelled data to further improve the student models.
% Beam sizes of 20 and 8 are used for w2v2-based models and Conformer-based model.

\presec
\subsection{KD for Non-Streaming Transducers}
\postsec
\label{ssec:non-streaming_trans}
Two KD training strategies are investigated for the proposed distillation loss. The first strategy (ST1) trains the student transducer model from scratch using \eqndot{kd full loss}. The second strategy (ST2) initialises the student model from a model trained on ground truth or pseudo transcriptions and then uses the proposed loss in \eqndot{kd full loss} for fine-tuning.
\begin{table}[ht]
    \pretbl
    \centering
    \begin{tabular}{lrrrr}
        \toprule
        \multirow{2}{*}{Transducer models}    & \multicolumn{2}{c}{dev}   & \multicolumn{2}{c}{test}  \\
        \cmidrule(lr){2-3}  \cmidrule(lr){4-5}
        & \multicolumn{1}{c}{clean} & \multicolumn{1}{c}{other} & \multicolumn{1}{c}{clean} & \multicolumn{1}{c}{other} \\ 
        \midrule
        \multicolumn{5}{l}{\textbf{Reference models: 100h labelled}}\\
        w2v2 transducer (teacher) & 5.1 & 12.2 & 5.2 & 11.8\\
        \rowcolor{LightCyan}
        Conformer-S (baseline)    & 7.5 & 20.9 & 8.0 & 21.8\\
        \midrule
        \multicolumn{5}{l}{\textbf{Student models: 100h labelled}}\\
        $\lambda=0.001$, collapsed \cite{panchapagesan2021fulllatticernntkd} & 7.1 & 20.7 & 7.5 & 20.9\\
        \rowcolor{LightCyan}
        $\lambda=0.001$, collapsed \cite{panchapagesan2021fulllatticernntkd}, ST2 & 6.8 & 19.2 & 7.2 & 19.8\\
        $\lambda=0.1$, ST1       & 7.1 & 19.8 & 7.6 & 20.5 \\
        \rowcolor{LightCyan}
        $\lambda=0.1$, ST2       & 6.7 & 19.0 & 7.1 & 19.3 \\
        \rowcolor{LightCyan}
        $\lambda=0.1$, ST2 [+LM] & 6.7 & 18.9 & 7.0 & 19.3 \\
        \midrule
        \multicolumn{5}{l}{\textbf{Student models: 100h labelled + 860h unlabelled}}\\
        $\lambda=0.0$            & 5.5 & 11.5 & 5.6 & 11.9 \\
        $\lambda=0.0$ [+LM]      & 4.7 & 10.4 & 4.8 & 10.9 \\
        $\lambda=0.1$, ST1       & 5.5 & 11.3 & 5.5 & 11.7 \\
        $\lambda=0.1$, ST2       & 5.3 & 10.9 & 5.4 & 11.3 \\
        $\lambda=0.1$, ST2 [+LM] & 4.6 & 10.1 & 4.8 & 10.4 \\
        \bottomrule
    \end{tabular}
    \caption{WERs of non-streaming transducer models. $\lambda$ is the weight of KD loss. [+LM] means either the teacher output distributions or the pseudo transcriptions are obtained after LM shallow fusion.}
    \label{tab:non-streaming KD}
    \posttbl
\end{table}
% KD experiments are first carried out on non-streaming transducer models.
% For ST2, we initialise the model from baseline model in \tbl{ref models} in 100h experiments and the model trained with 100h ground truth and 860 pseudo transcription data in 960h experiments.
% ST1 means the student model is trained from scratch. ST2 means the student model is initialised from a model trained on ground truth or pseudo transcriptions. 

Five key observations can be made from \tbl{non-streaming KD}.
First, for student models trained from 100h labelled data, the proposed distillation loss using the full distribution on the one-best alignment slightly outperforms KD using a collapsed distribution on the whole lattice~\cite{panchapagesan2021fulllatticernntkd}.
Secondly, for student models trained from 100h labelled data and 860h unlabelled data, the proposed KD method yields lower WERs than simply using the pseudo transcriptions ($\lambda=0.0$) for the unlabelled data because the output distribution carries more information from the teacher to the student than the pseudo transcriptions.
Thirdly, ST2 has lower WERs than ST1 for both the 100h and the 960h setups. As a result, ST2 will be used for the streaming experiments in \ssectdot{streaming_trans}.
Fourthly, the relative WER reductions (WERRs) on test-clean and test-other are \textcolor{blue}{11.3\% and 11.5\%} by using the proposed KD loss compared with the baseline. They increase to \textcolor{blue}{32.5\% and 48.2\%} when an additional 860h of unlabelled data is used for KD.
Lastly, to distil the knowledge from both the teacher model and the LM together, shallow fusion is used to generate the pseudo transcriptions on the unlabelled data and to augment the output distributions. This leads to WERRs of \textcolor{blue}{12.5\% for the 100h setup compared with the baseline on test-clean}. After incorporating 860h unlabelled data, the \textcolor{blue}{WERRs on test-clean and test-other improve to 40.0\% and 52.3\%}.

% To prevent model from diverging and catastrophic forgetting, the fine-tuning learning rate in ST2 is set very small.
%Note that the student model pre-training in the second strategy is only performed on clean-100h dataset to ensure only limited resource of labelled data is used. 
% In clean-100h experiments, the result of our implementation of \cite{panchapagesan2021fulllatticernntkd} is also included for comparison. For 960h experiments, the pseudo transcriptions decoded from the teacher transducer model and one-best path of 860h unlabelled data are collected. The WERs are shown in \tbl{non-streaming KD}. Among the two KD training strategies, ST2 yields a better results in both 100h and 960h experiments, showing the necessity of a good initialisation for KD. Therefore, only ST2 will be adopted in the following experiments. Compared with results of the distillation loss in~\cite{panchapagesan2021fulllatticernntkd}, our method achieves a higher WER reduction on the more challenging other sets. Compared with the baseline student conformer models, a relative WER reduction of 12.8\% and 11.4\% can be observed on test-clean and test-other using our proposed distillation loss together with ST2 on clean-100h. 

% After including more unlabelled data, the performance gap between the teacher model and the student model is further closed. By fine-tuning the model trained with 100h ground truth and 860h pseudo transcription without KD, our distillation proposal further improves the WER, achieving a relative reduction of 37.2\% and 50.4\% (see bottom row in \tbl{non-streaming KD}) compared to the baseline model. We also see that the WER improvement brought by KD is less obvious in 960h experiments than in 100h experiments. This is due to the reason that the teacher model is only trained on clean-100h, thus the quality of both the pseudo transcription and one-best distillation label is limited. A further WER improvement is observed after incorporating LM information in the distillation label.

\presec
\subsection{KD for Streaming Transducers}
\postsec
\label{ssec:streaming_trans}
% ST2 means the student model is initialised from a model trained on ground truth or pseudo transcriptions. [+LM] means either the output distributions or the pseudo transcriptions are obtained after LM shallow fusion.
By introducing the parameter $\tau$ for delaying the alignment, the proposed one-best distillation loss is applied to train streaming student models.
% The modified one-best distillation loss is then applied to streaming transducer models. To ensure that no future information is used during prediction, the original Conformer block is modified. An attention mask is added to remove the contribution of future frames when calculating the attention score and the 1D-convolution is changed to 1D causal convolution to only attend to previous frames \cite{oord2016wavenet}.
As before, the distillation targets are still generated from the non-streaming teacher w2v2 transducer. When the streaming student model is trained to match the alignment of the non-streaming teacher, \ie when $\tau=0$, the WERs of the student model is even higher than the baseline due to a lack of future context. After observing the one-best alignment of a streaming transducer can be multiple steps behind the one-best alignment of a non-streaming transducer, the WERs of $\tau=6$ and $\tau=7$ (equivalent to a look-ahead of 240 ms and 280 ms) are shown in \tbl{streaming KD}. Although more delay steps result in improved WERs, the latency of the ASR model is also increased. Nevertheless, setting a sensible value of $\tau$ is key to train a student model using KD.
% Three $\tau$s of 0, 6 and 7 are experimented after observing the delay of posterior peak between w2v2 transducer and streaming student models in 100h experiments. WER results are shown in \tbl{streaming KD}. As expected, the KD results are very sensitive to the selection of $\tau$. The lowest WERs are obtained using $\tau=7$, which is also around the average delay of posterior peak between teacher and student lattice. Interestingly, if no time-shift is applied (i.e $\tau$=0), the student model after KD performs much worse than the streaming baseline. This again proves the significance of time-shift operation in streaming transducer distillation.
Compared with the streaming baseline, the proposed distillation approach achieves WERRs of 7.4\% and 6.8\% on test-clean and test-other in 100h experiments. After using the additional 860h unlabelled data, the student model trained with KD outperforms the one only trained with pseudo transcriptions, which increases WERRs to 19.7\% and 38.5\% \wrt the streaming baseline.
%After using the LM-augmented distillation targets, the WERs of the streaming student transducer are \% and \% lower than the baseline.
\begin{table}[ht]
    \pretbl
    \centering
    \begin{tabular}{lrrrr}
        \toprule
        \multirow{2}{*}{Transducer models}    & \multicolumn{2}{c}{dev}   & \multicolumn{2}{c}{test}  \\
        \cmidrule(lr){2-3}  \cmidrule(lr){4-5}
        & \multicolumn{1}{c}{clean} & \multicolumn{1}{c}{other} & \multicolumn{1}{c}{clean} & \multicolumn{1}{c}{other} \\ 
        \midrule
        \multicolumn{5}{l}{\textbf{Reference models: 100h labelled}}\\
        w2v2 transducer (teacher) &  5.1 & 12.2 &  5.2 & 11.8\\
        Conformer-S (baseline)         & 11.2 & 28.4 & 12.2 & 29.6\\
        \midrule
        \multicolumn{5}{l}{\textbf{Student models: 100h labelled}}\\
        $\lambda=0.1$, $\tau$=0, ST2 & 20.2 & 39.7& 20.5 & 41.4 \\
        $\lambda=0.1$, $\tau$=6, ST2 & 10.7 & 26.7& 11.3 & 28.0 \\
        $\lambda=0.1$, $\tau$=7, ST2 & 10.6 & 26.4& 11.3 & 27.6\\
        % $\lambda=0.1$, $\tau$=7, ST2 [+LM] & 10.4 & 26.5 & 11.1 & 27.4 \\
        \midrule
        \multicolumn{5}{l}{\textbf{Student models: 100h labelled + 860h unlabelled}}\\
        $\lambda=0.0$                & 9.5  & 19.3 & 10.6 & 19.7  \\
        % $\lambda=0.0$ [+LM]          & 9.1  & 18.4 & 10.3 & 18.5 \\
        $\lambda=0.1$, $\tau$=7, ST2 & 9.2  & 18.3 & 9.8  & 18.2 \\
        % $\lambda=0.1$, $\tau$=7, ST2 [+LM] & 8.9 & 18.7 & 9.7 & 18.7 \\
        \bottomrule
    \end{tabular}
    \caption{WERs of streaming transducer models. $\lambda$ is the weight of KD loss. $\tau$ is the number of delayed steps for the one-best alignment from the teacher model.}
    \label{tab:streaming KD}
    \posttbl
\end{table}
% [+LM] means either the output distributions or the pseudo transcriptions are obtained after LM shallow fusion.

% Although the streaming student has a much lower baseline than the non-streaming student, the relative improvement for the streaming student model is less. 


==> text_prev/intro.tex <==
\presec
\section{Introduction}
\postsec
Self-supervised learning has emerged as a paradigm to learn general data representations. The model is first pre-trained on a vast amount of unlabelled data and then fine-tuned with some task-specific labelled data. % to perform downstream tasks.
The effectiveness of this approach was first demonstrated in various natural language processing tasks~\cite{devlin2018bert,brown2020GPT3} and, more recently, in automatic speech recognition (ASR)~\cite{baevski2019vqw2v2,baevski2020wav2vec}.
% Recently, the idea of self-supervised learning has also been adopted in ASR. By extensive pre-training on untranscribed speech data, the model is then fine-tuned with transcribed speech data to perform ASR tasks~\cite{baevski2020wav2vec,baevski2019vqw2v2}. 
Promisingly, some of these models could reach state-or-the-art performance without relying on a large amount of labelled data.
% Promisingly, these models have shown state-or-the-art results while requiring much less labelled data.
Although self-supervised pre-training exhibits compelling performance for ASR, the models are typically very large with hundreds of millions or even billions of parameters. This leads to large memory consumption and long inference time, which hinders the direct deployment of such models for real-world ASR applications~\cite{peng2021shrinking}. Moreover, the pre-trained speech encoder is generally bidirectional or attends to a very wide range of past and future context~\cite{baevski2020wav2vec,baevski2019vqw2v2}, which is prohibitive for ASR applications that require streaming processing of speech data.
% Despite the advantages of the self-supervised ASR models, they are typically very large in size. The fine-tuned models tend to have hundreds of millions of parameters, leading to long inference time and large memory consumption. This property prevents them to be adopted in real ASR applications such as on-device speech recognition.

To this end, various model compression methods have been proposed in the past to reduce the model size dramatically without hurting the performance significantly. For example, singular value decomposition on weight matrices can reduce the number of parameters of acoustic models for feedforward networks~\cite{xue2013restructuring} and recurrent neural networks (RNNs)~\cite{prabhavalkar2016compression}, sparse pruning method shrinks the model size by setting weights with small values to zero~\cite{zhen2021sparsification}.
% Thus, methods that compress models without significantly affecting the performance are needed before the self-supervised ASR models can be applied. In \cite{xue2013restructuring}, singular value decomposition (SVD) was applied to restructure the original acoustic model, leading to a much smaller ASR model. With an extra fine-tuning step, no performance degradation is observed at a 35\% model size reduction. A similar idea is also adopted in \cite{prabhavalkar2016compression} and achieves good compression performance on recurrent neural networks. In \cite{zhen2021sparsification}, a sparse-aware pruning method is applied during the feed-forward process to compress an RNN-transducer model \cite{graves2012RNNT} and achieves little performance reduction at a sparsity ratio of 50\%. 
Instead of direct manipulation of model parameters, knowledge distillation (KD)~\cite{hinton2015knowledgedistillation} is an alternative for model compression, where a small student model learns to mimic the output behaviour of a large teacher model. As KD only depends on the outputs from the teacher and student models, the student model is free to have a different representation of the input data and also a different model architecture. KD is also able to take advantage of unlabelled data as only the output from the teacher model is needed to train the student model~\cite{cao2021improving, doutre2021improving}. For conventional hidden Markov model-based systems, KD has been applied to the acoustic model at the frame level~\cite{Li2014LearningSD} or the sequence level~\cite{Wong2016SequenceST}. For end-to-end (E2E) ASR, KD has been applied for connectionist temporal classification (CTC) models~\cite{takashima2018ctcseqkd, kurata2018improvedCTCkd, takashima2019investigationCTCseqkd,Yoon2021TutorNetTF} and attention-based encoder-decoder models~\cite{2018CompressionLAS,Yoon2021TutorNetTF} by either matching the hidden representations or the softmax output distributions between the teacher and student models. Neural transducer~\cite{graves2012RNNT} is another widely adopted E2E ASR model because of its competitive performance and readiness for streaming applications~\cite{rao2017exploring, he2019streaming}. However, applying KD on transducers is less straightforward as computing the distillation loss on the whole output probability lattice from transducers is very expensive and memory-inefficient, especially for long sequences. \cite{doutre2021improving} trained the student transducer model directly from the ``pseudo transcriptions'', \ie erroneous recognition results of the teacher model, instead of using the output distributions. \cite{panchapagesan2021fulllatticernntkd} carried out the KD for transducers using a collapsed version of the full output distributions to reduce the memory requirement during training. As a workaround, \cite{swaminathan2021codert} performs KD over the encoder hidden representations.
% Knowledge distillation (KD) is another popular choice of compressing ASR models for on-device applications. The distillation process involves a teacher model and a student model, where the student model attempts to mimic the teacher model's output behaviour.
% Different from other compression methods, KD poses fewer requirements on the model architecture selection as it does not address the learning problem from the weight perspective. This allows KD to have the advantage of utilising unlabelled data as extra training data since only the output of the teacher model is relevant to the student model training~\cite{cao2021improving, doutre2021improving}.
% In \cite{takashima2018ctcseqkd, kurata2018improvedCTCkd, takashima2019investigationCTCseqkd}, KD is applied under CTC architecture to improve ASR performance. Similar ideas have been applied to attention-based architectures~\cite{2018CompressionLAS} and showed promising results.
% Among all the modern E2E ASR architectures, RNN-Transducer (RNN-T) model~\cite{graves2012RNNT} attracts the most attention due to its good performance and the natural support of streaming application~\cite{rao2017exploring, he2019streaming}. However, there has been no unified KD approach for RNN-T models due to its more complicated working mechanism and large memory consumption. Previous works mainly focus on improving streaming RNN-T models' performance by distilling knowledge from a non-streaming teacher RNN-T ~\cite{doutre2021improving, kurata2020knowledge}. In \cite{panchapagesan2021fulllatticernntkd}, RNN-T KD is carried out by minimising the sum KL-divergence calculated from a collapsed distribution over the teacher and student output lattice to reduce memory cost during training. In \cite{swaminathan2021codert}, distillation over the encoder feature output is adopted as another workaround. However, both methods result in information loss either by using a collapsed distribution of an intermediate representation for distillation loss calculation, which could limit the KD performance.

In this paper, we investigate how to effectively distil knowledge from a large pre-trained transducer model to a much smaller one with a limited amount of labelled data. Instead of using the collapsed distribution over the whole probability lattice~\cite{panchapagesan2021fulllatticernntkd}, using the full distribution of the one-best path in the output probability lattice yields better performance. The proposed distillation loss can be simply adapted to transfer knowledge from a non-streaming teacher to a streaming student by introducing a time-shift variable that controls the amount of future context seen by the encoder.
% In this work, we study how to distil knowledge from a large self-supervised ASR transducer model to a smaller transducer model, so that the small model is also able to yield good performance when only a limited amount of labelled data is available.
% To achieve this, we propose a novel distillation loss utilising the one-best path information in the output lattice for transducer models, which is both memory-efficient and effective. Then, we modify our distillation loss for application on streaming transducer models by introducing a time-shift variable to address the different emission behaviours of streaming and non-streaming transducer models.
In our experiments, the teacher is a wav2vec 2.0 model~\cite{baevski2020wav2vec} with the waveform as input, whereas the student is a Conformer model~\cite{gulati2020conformer} with filter bank features as input. Although the student model is 10 times smaller than the teacher model, experiments on LibriSpeech show that the proposed method significantly improves the student's performance for both non-streaming and streaming cases.
Further word error rate (WER) reduction is observed by using unlabelled data for KD or augmenting the distillation targets by a language model (LM).
% In particular, relative WER reductions of 50.4\% for non-streaming transducer and 38.5\% for streaming transducer on test-other set are achieved using 100h labelled data and 860h unlabelled data compared to the baseline model trained without KD. 

In the rest of this paper, \sectdot{background} briefly reviews self-supervised pre-training for ASR and the neural transducer models. In \sectdot{method}, the proposed distillation loss for streaming and non-streaming transducers are introduced.
Experimental setups and results are described in \twosectdot{setup}{results}. Conclusions are drawn in \sectdot{conclusion}.
% Experimental setups are described in \sectdot{setup} and then the speech recognition results are given in \sectdot{results}. Finally, conclusions are drawn in \sectdot{conclusion}

==> text_prev/method.tex <==
\presec
\section{Knowledge Distillation for Transducers}
\postsec
\label{sec:method}
% Here, we introduce our distillation loss proposal and compare it with existing RNN-T KD methods. In the end, we discuss the extension of our proposed distillation loss from two perspective: language model (LM) shallow fusion and streaming application.

Knowledge distillation (KD)~\cite{hinton2015knowledgedistillation} is a widely used model compression technique that trains a small student model to match the output of a large teacher model.
% Knowledge distillation~\cite{hinton2015knowledgedistillation}, or teacher-student training, is a commonly used model compression technique that can construct a high-performing student model by transferring knowledge from a teacher model. Instead of training the student model with ground truth data, the student model attempts to mimic the teacher model's output. This characteristic leads to KD's capability of utilising unlabelled data for student model training. 
In a classification task with $K$ classes, KD is usually carried out by minimising the Kullback–Leibler (KL) divergence as \eqndot{KL-divergence} between the teacher output distribution $p_{\mathcal{T}}$ and the student output distribution $p_{\mathcal{S}}$,
\begin{align}
    \mathcal{L}_{\text{KD}}=-\sum_{k=1}^{K} p_{\mathcal{T}}(k) \log \frac{p_{\mathcal{S}}(k)}{p_{\mathcal{T}}(k)}.
    \label{eqn:KL-divergence}
\end{align}
%If $p_{\mathcal{T}}$ is fixed during training, the last term in \eqndot{KL-divergence} can be ignored and the loss become the cross-entropy between $p_{\mathcal{T}}$ and $p_{\mathcal{S}}$.

Since it does not require ground truth labels, KD can leverage unlabelled data for student model training. KD also provides a greater extent of flexibility for model compression as it does not constrain the input features or the model architectures of the teacher and student models to be the same. 
% Since the output layer of E2E ASR models is , the teacher output distribution is a prevalent distillation target in KD and the distillation loss is usually used as an auxiliary loss to guide student model training~\cite{}.

\presec
\presec
\subsection{KD for Non-Streaming Transducer}
\postsec
\label{ssec:non-streaming}
As described in \sectdot{rnnt}, a transducer generates an output distribution lattice $\mathbf{Z}$ from a sequence acoustic features $\mathbf{X}$ and a label sequence $\mathbf{y}$, from which the total conditional probability of the label sequence given the acoustic sequence can be computed by summing over all possible alignments. Therefore, the output lattice of a teacher transducer is an obvious distillation target for the student model. A straightforward implementation of distillation loss would be the KL divergence (or cross-entropy as the teacher labels are fixed) between the output distribution lattices of the student $\mathbf{Z}_{\mathcal{S}}$ and teacher $\mathbf{Z}_{\mathcal{T}}$ as in \eqndot{fulllatticeKD}. As a result, the output distribution of the student model should imitate the teacher distribution over the entire lattice. However, this method is impractical due to its large memory and computation complexities of $\mathcal{O}(KTU)$.% as the whole teacher lattice needs to be loaded in the GPU during KD training. This prevents training in reasonable batch size and requires large computation resources.
\begin{align}
    \mathcal{L}_{\text{KD}} = -\sum_{t=1}^{T}\sum_{u=1}^{U}\sum_{k=1}^{K} \mathbf{Z}_{\mathcal{T}}(k,t,u) \log \mathbf{Z}_{\mathcal{S}}(k,t,u).
    \label{eqn:fulllatticeKD}
\end{align}

To reduce the computational cost of KD for transducers, distillation based on a collapsed distribution of all nodes in the lattice was proposed~\cite{panchapagesan2021fulllatticernntkd}. By only considering the blank symbol, the correct output symbol and all the remaining symbols, the output distribution on each node is reduced from $K$ to only 3 classes. The complexity becomes $\mathcal{O}(3TU)$.
% Therefore, the last summation is reduced from $K$ to $3$, leading to a much more memory-efficient loss calculation 
However, this method ignores the correlation across different output symbols compared to \eqndot{fulllatticeKD}, which could be important for training the student model using KD.

To achieve memory efficiency and also preserve the full distribution, we propose to distil knowledge only over the one-best path in the lattice instead of over the whole lattice. It has been shown that only a small proportion of nodes in the lattice contribute to the final decoding results~\cite{jain2019rnntconstrainedbm}, which indicates that a large number of paths in the lattice have low probabilities.
% In other words, the student model can only pay attention to the most important nodes in the lattice during KD.
As an approximation, only the nodes along the one-best path are considered as important. The distillation loss for one-best path in the output distribution lattice is: 
\begin{align}
    \mathcal{L}_{\text{KD}} \approx -\sum_{(t,u)\in \textsc{1Best}}\sum_{k=1}^{K} \mathbf{Z}_{\mathcal{T}}(k,t,u) \log \mathbf{Z}_{\mathcal{S}}(k,t,u),
    \label{eqn:rnnt onebest}
\end{align}
where $\textsc{1Best}$ is the most likely alignment between $\mathbf{X}$ and $\mathbf{y}$ containing the blank symbol. For an input utterance of length $T$ and a target sequence of length $U$, the memory complexity is only $\mathcal{O}(K(T+U))$. Compared with \cite{panchapagesan2021fulllatticernntkd}, the proposed approach preserves the full distribution for each node at the expense of ignoring other possible alignments. Assuming the probability lattice is relatively sparse, the proposed method is expected to transfer richer information than the collapsed distribution~\cite{panchapagesan2021fulllatticernntkd}. Furthermore, using the one-best alignment allows the alignment to be delayed when training a streaming student from a non-streaming teacher as discussed in \ssectdot{streaming}.

\presec
\subsection{KD for Streaming Transducer}
\postsec
\label{ssec:streaming}
In contrast to non-streaming transducers, directly applying one-best KD as in \eqndot{rnnt onebest} to streaming transducers may not be sensible. As little (or no) future context is available for a streaming transducer, it tends to emit symbols later than non-streaming models to gather more future information~\cite{kurata2020knowledge}.
In other words, the most likely alignment for a streaming transducer normally lags behind its non-streaming counterpart by several time steps.
% Therefore, the posterior peak in the non-streaming model's lattice is usually delayed by several time stamps compared to its streaming counterpart.
As the pre-trained teacher model is non-streaming, directly applying \eqndot{rnnt onebest} to perform KD on a streaming student model may force the student model to ``guess'' into the future, which may lead to poor performance.
%emit symbols as early as the teacher model by matching the teacher's posterior peak, which can be problematic.
To this end, a hyperparameter $\tau$ is introduced to delay the non-streaming alignment, which allows the student model to emit symbols $\tau$ frames later than its teacher. $\tau$ can be tuned to find the best trade-off between performance and latency. To train a streaming student model, the modified distillation loss is 
% To handle the mismatch of posterior peak, we introduce an adjustable time shift factor $\Delta T$ to allow the student model to emit symbol later by $\Delta T$ time stamp.
% This leads to a modified version of one-best distillation loss for non-streaming transducers:
\begin{align}
    \mathcal{L}_{\text{KD}} \approx -\sum_{(t,u)\in \textsc{1Best}}\sum_{k=1}^{K} \mathbf{Z}_{\mathcal{T}}(k,t,u) \log \mathbf{Z}_{\mathcal{S}}(k,t+\tau,u).
    \label{eqn:rnnt onebest streaming}
\end{align}

\presec
\subsection{Using Unlabelled Data and LM Fusion for KD}
\postsec
Unlike other model compression techniques, KD is a data-driven approach that is able to leverage unlabelled data to further improve the student model. For unlabelled speech data, the teacher model is used to generate one-best hypotheses via beam search. The one-best alignment and the output probabilities of each node on it for each utterance are used as distillation targets.

During decoding, an external language model (LM) can be used to improve the quality of the transcription~\cite{bahdanau2016end, kannan2018analysis}, which is beneficial to KD training. %Despite the improved recognition performance, LM increases the complexity of a E2E ASR model. Previous work minimised the KL-divergence between the LM output distribution and E2E ASR model output distribution to incorporate LM information during training~\cite{bai2019learn}. 
In this work, the log-linear interpolation (shallow fusion)~\cite{bahdanau2016end} of transducer and an external LM is adopted to construct distillation targets containing LM information:
%as  The distillation targets after shallow fusion with an LM becomes
\begin{align}
    \mathbf{Z}'_{\mathcal{T}}(t, u) = \log(\textsc{Softmax}(\mathbf{Z}_{\mathcal{T}}(t,u))+\beta\log(\textsc{LM}(t)),
\end{align}
where $\textsc{LM}(t)$ is a $K$-dimensional vector representing the LM output distribution given the previously predicted sequence before $t$ and $\beta$ is a tuned LM weight. Note that the LM score for the blank symbol is set to zero when the blank symbol is emitted and $\min(\text{LM}(t))$ when a non-blank symbol is emitted. %Different from ~\cite{bai2019learn}, this choice of distillation target 
For a better convergence, the distillation loss is interpolated with the original transducer loss,
\begin{align}
    \mathcal{L} = \mathcal{L}_{\text{transducer}} + \lambda \mathcal{L}_{\text{KD}},
    \label{eqn:kd full loss}
\end{align}
where $\lambda$ is the interpolation coefficient.
% Our one-best distillation loss can also be easily extended to utilise un-transcribed speech data, which is also one of KD's merits compared to other neural network compression techniques. For un-transcribed speech data, pseudo transcription can be first generated with beam search decoding base using the teacher model. To reduce the computation complexity, the alignment $\mathbf{h}$ with the highest probability found with fixed-size beam search is then selected as the ``one-best'' path for the distillation loss calculation by keeping the distribution producing each symbol (including $\varnothing$) in $\mathbf{h}$. Note that the beam search decoding process can include a language model to improve the pseudo transcriptions' quality. Consequently, the distribution generating each symbol in $\mathbf{h}$ is also modified to incorporate LM information. This fusion is done in the logit space:
% \begin{align}
%     z'_t = \log(\textsc{Softmax}(z_t(t,u)))+\beta\log(\textsc{Softmax}(\text{LM}(t)))
% \end{align}
% where $LM(t)$ is a $K$-dimensional vector representing the LM prediction given the previous predicted sequence before $t$ and $\beta$ is a tuned LM weight. After generating the pseudo transcription and the distribution along the one-best path, \eqndot{rnnt onebest} and \eqndot{rnnt onebest streaming} can be applied to non-streaming and streaming models respectively.

% Finally, the distillation loss is combined with the original transducer loss to form the actual loss function:
% \begin{align}
%     L = L_{\text{RNN-T}} + \lambda L_{\text{KD}}
% \end{align}
% where $\lambda$ is a tuneable parameter controlling the contribution of distillation loss. In this way, our KD strategy can be treated as an auxiliary task during transducer training.





==> text_prev/rebuttal_1.tex <==
```
This paper proposes to use knowledge distillation (KD) for large pre-trained ASR models like wav2vec in order to improve the accuracy of smaller deployable models. The topic is of very practical interest in the ASR research community. The specific deployable model chosen here is a neural transducer (NT) with a Conformer acoustic encoder. The main contribution of the paper is to use the scores over the 1-best path in the NT output lattice for KD. The paper is well written with a clear coherent style of developing the main ideas and supporting them with evidence. 

I subscribe to the basic premise of the authors that the proposed method of KD through the 1-best path for NT is better than the earlier proposed method of collapsed distributions. It would have better if there was supporting evidence in the paper as that would have made the paper more complete. 

Overall, I would say that the paper is clearly among the better papers we see at ICASSP.
```

Dear reviewer,

Thank you for for reviewing our paper and providing constructive feedback.

We think the main advantage of our 1-best path knowledge distillation method comes from the richer information carried in the full distribution. With the earlier method using a collapsed distribution, we can quantify the information loss by calculating the change in entropy after collapsing the full distribution. A significant entropy drop would further justify our proposed method. We will carry out this experiment and consider adding this evidence to the final version.

% #TODO:
% The reviewer buys your idea of using 1-best over collapsed distribution, but he/she wants to see some evidence apart from the final WERs that justifies the claims such as "richer distribution" and "most of the paths are not important". For example, you can try to say, for example, measure the entropy of output distribution (except correct and blank) to verify that full distribution is important; similarly, we can measure the posterior of 1-best path over all paths to verify that 1-best dominate the output lattice.

% We agree that the manuscript would have been more convincing if more evidence is listed to support the superiority of our 1-best path knowledge distillation (KD) method over the collapsed distribution KD method. Here, we would like to emphasise the benefits of our 1-best path knowledge distillation (KD) method again from the following aspects:

% \begin{enumerate}
%     \item Compared to the collapsed distribution KD method, our method preserves the full distribution along the 1-best path while removing the less useful nodes in the lattice. Although the neural transducer (NT) output lattice is able to flexibly model all alignments between input acoustic frames $\mathbf{x}_{1:T}$ and output token sequence $y_{1:U}$, a large number of paths still have low probabilities if they pass through nodes $(t,u)$ generated by mismatched pair $\mathbf{x}_t$ and $y_u$ (especially at the edge of the lattice). Since the collapsed distribution KD treats each node in the lattice equally, we could argue that only a small proportion of the KD loss facilitates the student model training. On the contrary, our KD loss function spares the computation effort on less useful nodes and focuses on the full distribution of nodes on the 1-best path. As a full distribution contains richer information than the 3-element collapsed distribution, our KD method was able to further improve the student model.
    
%     \item Another unmentioned benefit of our KD method is the memory efficiency when $T$ and $U$ are large. Our method has a linear space complexity $\mathcal{O}(K(U+T))$ ($K$ is the vocabulary size) whereas the collapsed distribution method is $\mathcal{O}(UT)$. Also, our method can be easily extended to distil knowledge over n-best paths to transfer more knowledge from the teacher model.
    
% \end{enumerate}



% The full distribution carries richer information and leads to larger performance improvement. On the contrary, the collapsed distribution only contains three elements: the blank symbol, the correct output symbol and the sum of the rest symbols.  In the collapsed distribution KD training, the actual output symbols of such nodes are merged with the rest symbols, resulting in the loss of information after the computation of KL-divergence. Therefore, imitating the teacher's output behaviour on such nodes is likely to have little improvement of the student model's decoding accuracy. Our method ignores the less important paths and only focuses on the 1-best alignment. As can be seen from \autoref{tab: different beam size}, the one-best decoding results are only slightly worse than the best decoding results.
    
%     \begin{table}[h]
% \centering
% \begin{tabular}{lcccc}
% \toprule
% \multirow{2}{*}{Teacher w2v2 transducer model}    & \multicolumn{2}{c}{dev}   & \multicolumn{2}{c}{test}  \\
% \cmidrule(lr){2-3}  \cmidrule(lr){4-5}
% & \multicolumn{1}{c}{clean} & \multicolumn{1}{c}{other} & \multicolumn{1}{c}{clean} & \multicolumn{1}{c}{other} \\ 
% \midrule
% beam size 8 & 5.1 & 12.2 &  5.2  & 11.8\\
% beam size 1 & 5.3 & 12.6 &  5.4 & 12.1\\

% \bottomrule
% \end{tabular}
% \caption{WERs of the teacher w2v2 transducer model decoded with beam size 8 and 1 (greedy decoding).}
% \label{tab: different beam size}
% \end{table}

==> text_prev/rebuttal_2.tex <==
```
The paper proposes a simple and efficient knowledge distillation loss function for neural transducers with a full distribution along the 1-best alignment of the output distribution lattice. It is a well-written paper with convinced technique details and experimental results.
```

Dear reviewer,

Thank you for for reviewing our paper and we sincerely appreciate your kind comments.

==> text_prev/rebuttal_3.tex <==
```
This is a solid paper. In Table 2, what is the WER for the conformer\_s model trained on the full 960 transcribed audio, this can be served as a good reference point.
In Table 4, what about knowledge distillation with LM on? Does that help here?
```
Dear reviewer,

Thank you for for reviewing our paper and providing constructive feedback on our experiments.

We would like to ensure that all the results are comparable in our tables. In Table 2, all of the models are trained using 100-hour labelled data. Therefore, we did not include the model trained on the full 960-hour labelled data set. We do agree that such a model is an interesting reference point and we will consider adding it into the description. A Conformer-S model achieves a WER of 2.7/6.3 on test-clean and test-other respectively according to the original Conformer paper [24]. Although different vocabularies are used, we expect the WERs to be similar in our case. 

In the streaming transducer experiments in Table 4, we observed a performance gain compared to the baseline models but only by a small extent after using LM fusion for generating distillation targets. In future work, we will investigate how to more effectively distil both transducer and LM knowledge together into a single student model.

% We thank again for your generous comments.

% #TODO
% You can start by saying that we would like to keep everything comparable within a table. In the case of Table 2, all models are trained using 100-hour labelled data. Then acknowledge that it would be an interesting reference point and we will consider add it to the description. You can refer to the conformer paper with respect to the 960h number.

% We agree that a Conformer-s model trained on full 960h transcribed audio would be a good reference point in Table 2. We did not include this model at the first place as the goal of our work is to see how much a student conformer model could benefit from a w2v2 teacher model under the framework of knowledge distillation (KD) training. Therefore, we mainly focused on the performance improvement of the student models trained with KD compared to the baseline model trained without KD and the performance gap between them and the teacher model. We did not expect the model to match student model trained with KD to match a conformer model trained on full 960h transcribed LibriSpeech data. However, such comparison would still be interesting to do as it provides another perspective showing the effectiveness of our KD method.\\

% # TODO
% It's better to say that we observed gain but to a smaller extent. We are still investigating how to more effectively distil both RNN-T and LM knowledge together into a single student model.

% About the absence of LM-fused KD training result in Table 4, this is an issue we are still investigating. We carried out some experiments using LM-augmented distillation labels and no obvious performance improvement has been observed. As we observed some instability during streaming transducer training, we are planning to do some modifications in the streaming transducer KD training to overcome this issue. One potential direction is to allow a flexible selection of number of delayed frames ($\tau$) during loss calculation. Then, we will evaluate the LM-fused KD training for streaming transducers again.\\


==> text_prev/setup.tex <==
\presec
\section{Experimental Setup}
\postsec
\label{sec:setup}

% \presec
\subsection{Model}
\postsec
For the teacher model, the base w2v2 model~\cite{baevski2020wav2vec} is used to initialise the encoder of a transducer model.
% The 960-hour LibriSpeech dataset~\cite{} is used for pre-training and its 100-hour clean subset is used to fine-tune the teacher transducer model.
The original w2v2 model takes the waveform as input and has an output frequency of 100 Hz, whereas commonly used transducers have filter bank features as input and operate at 50 Hz. To achieve efficient knowledge distillation, a sub-sampling layer is added on top of the pre-trained model to reduce the frequency of the encoder output to 50 Hz. 
% In this work, we select the base w2v2 as teacher model. The base version of the w2v2 model \cite{baevski2020wav2vec} pre-trained on 960h-LibriSpeech dataset is used to initialise the encoder of an transducer model, which will be jointly fine-tuned with the decoder using labelled data. To reduce both memory cost and computation cost of knowledge distillation, we designed a sub-sampling module to reduce the encoder output frame-rate from 100Hz to 50Hz. This is achieved by first concatenating every two encoder output $\mathbf{z}_{2t}$ and $\mathbf{z}_{2t+1}$ and then adding a linear layer to resize back to the original dimension.
The student model is a small Conformer transducer model~\cite{gulati2020conformer}. Both models have a single-layer long short-term memory (LSTM) projection network. The output vocabulary has 256 subword units generated using SentencePiece~\cite{kudo2018sentencepiece}. The details of both models are given in \tbl{model comparison}.
The student model is more than 10 times smaller than the teacher model.
% We notice that a compression rate of 10.2 is achieved under our KD setup. Therefore, a significant performance degradation from the student model should be expected. However, this in turn leaves more space for potential performance improvement brought by K. 
For the LM used in shallow fusion, a 2-layer LSTM with 2048 units is trained from LibriSpeech LM corpus. The vocabularies of the transducer models and the LM are the same. All models are implemented in ESPnet~\cite{watanabe2018espnet}.
\begin{table}[ht]
    \pretbl
    \centering
    \begin{tabular}{ccc}
        \toprule
                & Teacher model & Student model \\
        \midrule
        Encoder & w2v2~\cite{baevski2020wav2vec} & Conformer-S~\cite{gulati2020conformer} \\
        Encoder dim & 768 & 144\\
        Decoder dim & 640 & 320 \\
        Num params & 99.2M & 9.7M\\
        \bottomrule
    \end{tabular}
    \caption{Details of the teacher and student transducer models.}
    \label{tab:model comparison}
    \posttbl
    \posttbl
\end{table}

\presec
\subsection{Data}
\postsec
LibriSpeech dataset~\cite{Panayotov2015LibrispeechAA} is used for the following experiments. The full training set has 960 hours of audiobook recordings. Among these, ``train-clean-100'' is used as labelled data while the remaining 860 hours are treated as unlabelled data. The teacher model is pre-trained using the full training set and fine-tuned on the 100-hour labelled subset following \cite{baevski2020wav2vec}.
% We evaluate the proposed distillation loss on the 960h LibriSpeech dataset. For teacher w2v2 model, the normalised waveform is used as input for fine-tuning the pre-trained model following the instructions in ~\cite{baevski2020wav2vec} with a tri-state adam optimiser. The 83-dimensional filter bank coefficients are used as input features for student models and noam optimiser ~\cite{vaswani2017transformer} is used for training. The amount of labelled data is limited to 100h in all experiments, while the rest 860h is treated as unlabelled dataset for the semi-supervised learning experiments. 
